Shock formation in 1D conservation laws I: Inviscid structure

We study the stability and structure of shock formation in 1D hyperbolic conservation laws. We show that shock formation is stable near shocking simple waves: perturbations form a shock nearby in spacetime. We also characterize the boundary of the classical development in a spacetime neighborhood of the first time singularity. Finally, we describe the precise nature of nondegenerate shock formation through an expansion in homogeneous functions of fractional degree. We use these results in a companion paper to study the vanishing viscosity limit near shock formation.

==> And-Cha-Gra-macros.tex <==
\newcommand*{\R}{\mathbb{R}}
\providecommand*{\C}{}
\renewcommand*{\C}{\mathbb{C}}
\newcommand*{\N}{\mathbb{N}}
\newcommand*{\Z}{\mathbb{Z}}
\newcommand*{\Q}{\mathbb{Q}}
\newcommand*{\T}{\mathbb{T}}
\newcommand*{\A}{\mathbb{A}}
\newcommand*{\E}{\mathbb{E}}
\newcommand*{\K}{\mathbb{K}}
\newcommand*{\F}{\mathbb{F}}
\newcommand*{\D}{\mathbb{D}}
\newcommand*{\Ham}{\mathbb{H}}
\newcommand*{\hs}{\mathbb{H}}
\renewcommand*{\P}{\mathbb{P}}
\newcommand*{\e}{\mathrm{e}}
\newcommand*{\cc}{\mathrm{c}}
\newcommand*{\eps}{\varepsilon}
\newcommand*{\al}{\alpha}
\newcommand*{\Om}{\Omega}
\newcommand*{\bd}{\partial}
\newcommand*{\h}[1]{\hat{#1}}
\newcommand*{\s}[1]{\mathscr{#1}}
\newcommand*{\m}[1]{\mathcal{#1}}
\newcommand*{\fr}[1]{\mathfrak{#1}}
\newcommand*{\dn}{\mathrm{d}}
\newcommand*{\diff}{\mathrm{d}}
\newcommand*{\ds}{\,\mathrm{d}}
\renewcommand*{\d}{\;\mathrm{d}}
\newcommand*{\Der}{\mathrm{D}}
\newcommand*{\der}[2]{\frac{\dn #1}{\dn #2}}
\newcommand*{\pa}[2]{\frac{\partial #1}{\partial #2}}
\newcommand*{\abs}[1]{\left |#1 \right|}
\newcommand*{\abss}[1]{|#1|}
\newcommand*{\absb}[1]{\big|#1\big|}
\newcommand*{\norm}[1]{\left \|#1 \right\|}
\newcommand*{\norms}[1]{\|#1\|}
\newcommand*{\normb}[1]{\big\|#1 \big\|}
\newcommand*{\braket}[1]{\langle #1 \rangle}
\newcommand*{\Braket}[1]{\left\langle #1 \right\rangle}
\newcommand*{\op}[1]{\operatorname{#1}}
\newcommand*{\sgn}{\op{sgn}}
\newcommand*{\ti}[1]{\tilde{#1}}
\newcommand*{\ubar}[1]{\underline{#1}}
\newcommand*{\tbf}[1]{\textup{\textbf{#1}}}
\newcommand*{\trm}[1]{\textup{\textrm{#1}}}
\newcommand*{\id}[1]{\op{id}_{#1}}
\newcommand*{\anon}{\,\cdot\,}
\renewcommand*{\Re}{\op{Re}}
\renewcommand*{\Im}{\op{Im}}
\newcommand*{\Ker}{\op{ker}}
\newcommand*{\Image}{\op{im}}
\newcommand*{\Span}{\op{span}}
\newcommand*{\supp}{\op{supp}}
\newcommand*{\trans}[1]{\tensor*[^t]{#1}{}}
\newcommand*{\smooth}[1]{\m{C}_c^\infty(#1)}
\newcommand*{\arccot}{\op{arccot}}
\newcommand*{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand*{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand*{\noorm}[1]{\left|\left \|#1 \right\|\right|}
\newcommand*{\MLoc}{\m M_{c,\text{loc}}}
\newcommand*{\BM}{Brownian motion~}
\renewcommand*{\And}{\quad \text{and} \quad}
\newcommand*{\For}{\quad \text{for }}
\newcommand*{\ForAll}{\quad \text{for all }}
\newcommand*{\nab}{\nabla}
\newcommand*{\trdeg}{\op{tr\,deg}}
\newcommand*{\gr}{\op{gr}}
\newcommand*{\rees}{\op{Rees}}
\newcommand*{\Spec}{\op{Spec}}
\renewcommand*{\hom}[2]{\op{Hom}(#1, #2)}
\renewcommand*{\div}{\op{div}}
\newcommand*{\bbraket}[1]{\left \langle \! \left \langle #1 \right \rangle \! \right \rangle}
\newcommand*{\power}[1]{{#1}[\![X]\!]}
\newcommand*{\laurent}[1]{{#1}(\!(X)\!)}
\DeclareMathOperator*{\Dlim}{D-lim}
\DeclareMathOperator*{\Clim}{C-lim}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\newcommand*{\mr}{\mathring}
\newcommand*{\smallO}{
  \mathchoice
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}%
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}%
    {\scalebox{.9}{$\scriptscriptstyle\mathcal{O}$}}%
    {\scalebox{.6}{$\scriptscriptstyle\mathcal{O}$}}%
  }

\newcommand{\sperp}{
{\mathchoice
{\mbox{\smaller$\bm\perp$}}
{\mbox{\smaller$\bm\perp$}}
{\mbox{\smaller[5]$\bm\perp$}}
{\mbox{\smaller[6]$\bm\perp$}}
}
}

\newcommand*{\iu}{\mathrm{i}}

\newcommand*{\smallbar}[1]{\overline{#1}}
\let\temp\bar
\let\bar\smallbar
\let\smallbar\temp
\let\temp\undefined

\newcommand*{\Hu}{\mathbb{H}}
\let\temp\H
\let\H\Hu
\let\Hu\temp
\let\temp\undefined

\newcommand*{\nsind}{\llbracket 2, N \rrbracket}

\newcommand*{\cub}{\fr{u}}
\newcommand*{\cubder}{\fr{m}}
\newcommand*{\dist}{\fr{d}}
\newcommand*{\Dist}{\fr{D}}
\newcommand*{\euc}{\fr{e}}
\newcommand*{\Euc}{\fr{E}}

\newcommand*{\out}[2]{{#1}_{#2}^{\textnormal{out}}}
\newcommand*{\inn}[2]{{#1}_{#2}^{\textnormal{in}}}
\newcommand*{\app}[2]{{#1}_{#2}^{\textnormal{app}}}
\newcommand*{\cut}[2]{{#1}_{#2}^{\textnormal{cut}}}
\newcommand*{\res}{{\textnormal{res}}}
\newcommand*{\match}{{\textnormal{m}}}
\newcommand*{\tb}{t_{\mathrm{b}}}
\newcommand*{\sft}{\mathsf{t}}
\newcommand*{\sfx}{\mathsf{x}}

\newcommand*{\Is}{{1}}
\newcommand*{\const}{\texttt{c}}
\newcommand*{\func}{\texttt{f}}
\newcommand*{\poly}{\mathsf{p}}

\newcommand*{\bigsub}[1]{{\mathclap{\substack{#1}}}\,}
\newcommand*{\Aop}{\m{A}}
\newcommand*{\Bop}{\m{B}}
\newcommand*{\Eta}{\mathsf{H}}
\newcommand*{\neweps}{\zeta}

\newcommand{\CG}[1]{{\color{green!60!black}\textbf{CG:} #1}}
\newcommand{\SC}[1]{{\color{red}\textbf{SC:} #1}}
\newcommand{\JA}[1]{{\color{blue} \textbf{JA:} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\green}[1]{{\color{green} #1}}

\newcommand*{\bR}{\mathbf{R}}
\newcommand*{\om}{\omega}
\newcommand*{\innind}{\s{I}}
\renewcommand*{\P}{\mathcal{P}}
\newcommand*{\inv}{{^{-1}}}
\newcommand*{\Ph}{\mathcal{P}}
\newcommand*{\Phs}{\Phi}
\newcommand*{\Phns}{\phi}
\newcommand*{\vbar}{\underline{v}}
\newcommand*{\half}{\frac 12}
\newcommand*{\ie}{i.\,e}
\newcommand*{\f}{\frac}
\DeclareMathOperator{\divr}{div}
\newcommand*{\fu}{\mathfrak{u}}
\newcommand*{\ft}{\mathfrak{t}}
\newcommand*{\fm}{\mathfrak{m}}
\newcommand*{\rd}{\partial}
\newcommand*{\fd}{\mathfrak{d}}
\renewcommand*{\D}{\mathcal{D}}
\newcommand*{\ls}{\lesssim}
\newcommand*{\gs}{\gtrsim}
\newcommand*{\calM}{\mathcal{M}}
\newcommand*{\calJ}{\mathcal{J}}
\newcommand*{\calB}{\mathcal{B}}
\newcommand*{\Php}{\bar{\Ph}}
\newcommand*{\Phsp}{\bar{\Phs}}
\newcommand*{\mup}{\bar{\mu}}
\newcommand*{\psip}{\bar{\psi}}
\newcommand*{\muT}{\hat{\mu}}
\newcommand*{\xiT}{\hat{\xi}}
\newcommand*{\xip}{\bar{\xi}}
\newcommand*{\bfd}{\mathbf{d}}
\newcommand*{\bfA}{\mathbf{A}}
\newcommand*{\bfr}{\mathbf{r}}
\newcommand*{\bfG}{\mathbf{G}}
\newcommand*{\PhT}{\hat{\Ph}}
\newcommand*{\PhsT}{\hat{\Phs}}
\newcommand*{\psiT}{\hat{\psi}}
\newcommand*{\AT}{\hat{A}}
\newcommand*{\rT}{\hat{r}}
\newcommand*{\lT}{\hat{l}}
\newcommand*{\XiT}{\hat{\Xi}}
\newcommand*{\calR}{\mathcal{R}}
\newcommand*{\calL}{\mathcal{L}}
\newcommand*{\calI}{\mathcal{I}}
\newcommand*{\calD}{\mathcal{D}}
\newcommand*{\calW}{\mathcal{W}}
\newcommand*{\taut}{\tilde{\tau}}
\newcommand*{\La}{\Lambda}
\newcommand*{\LaT}{\hat{\La}}
\newcommand*{\Lap}{\bar{\La}}
\newcommand*{\RT}{\hat{R}}
\newcommand*{\Rp}{\bar{R}}
\newcommand*{\PiT}{\hat{\Pi}}
\newcommand*{\Sigt}{\widetilde{\Sigma}}
\newcommand*{\Sigs}{\Sigma^*}
\newcommand*{\mus}{\mu^*}
\newcommand*{\calDt}{\widetilde{\calD}}
\newcommand*{\calDs}{\calD^*}
\newcommand*{\muts}{\tilde{\mu}^*}
\newcommand*{\Sigts}{\widetilde{\Sigma}^*}
\newcommand*{\calE}{\mathcal{E}}
\newcommand*{\ep}{\epsilon}
\newcommand*{\calQ}{\mathcal{Q}}
\newcommand*{\calN}{\mathcal{N}}
\newcommand*{\calG}{\mathcal{G}}
\newcommand*{\PG}{\calG}
\newcommand*{\PGT}{\hat{\PG}}
\newcommand*{\PGp}{\bar{\PG}}
\newcommand*{\calT}{\mathcal{T}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calS}{\mathcal{S}}
\DeclareMathOperator{\Lip}{Lip}
\newcommand*{\vb}{\vbar}
\newcommand*{\calV}{\mathcal{V}}
